Specification and Verification with the TLA+ Trifecta: TLC, Apalache, and TLAPS

Using an algorithm due to Safra for distributed termination detection as a running example, we present the main tools for verifying specifications written in TLA+. Examining their complementary strengths and weaknesses, we suggest a workflow that supports different types of analysis and that can be adapted to the desired degree of confidence.

==> Makefile <==
TARGET=paper
SOURCE=paper

DEPS=$(TARGET).tex *.tex paper.bib llncs.cls splncs04.bst #fig/*.* 

REV:=set-revision-in-command-line
TMP:=$(shell mktemp -d /tmp/tmpdiff.XXXXXXXX)

all: $(TARGET).pdf

draft: draft.pdf

draft.pdf: draft.tex $(DEPS)
	pdflatex draft
	bibtex draft
	pdflatex draft
	pdflatex draft

diff: 
	# use REV=xxx make -e diff
	./latexpand.pl $(TARGET).tex >unrolled.tex
	echo $(TMP)
	cd $(TMP); svn co -r $(REV) $(shell svn info | grep "URL: " | sed 's/URL: \(.*\)/\1/g') .; \
		$(realpath $(@D))/latexpand.pl $(TARGET).tex >unrolled.tex
	latexdiff $(TMP)/unrolled.tex unrolled.tex >diff.tex
	pdflatex diff
	bibtex diff
	pdflatex diff
	pdflatex diff
	rm -rI $(TMP)

snapshot: main.pdf $(DEPS)
	tar cvzf snapshot.tgz main.pdf 

source: $(DEPS)
	tar cvzf source.tgz $(DEPS) main.bbl
	zip source.zip $(DEPS) main.bbl

$(TARGET).pdf: $(TARGET).tex $(DEPS)
	pdflatex $(TARGET)
	bibtex $(TARGET)
	pdflatex $(TARGET)
	pdflatex $(TARGET)

clean:
	rm -rf $(TARGET).pdf $(TARGET).aux $(TARGET).bbl $(TARGET).blg *~  draft.pdf draft.aux draft.bbl draft.blg $(TARGET).out $(TARGET).log draft.out draft.log

